Synthetic Photovoltaic and Wind Power Forecasting Data

Photovoltaic and wind power forecasts in power systems with a high share of renewable energy are essential in several applications. These include stable grid operation, profitable power trading, and forward-looking system planning. However, there is a lack of publicly available datasets for research on machine learning based prediction methods. This paper provides an openly accessible time series dataset with realistic synthetic power data. Other publicly and non-publicly available datasets often lack precise geographic coordinates, timestamps, or static power plant information, e.g., to protect business secrets. On the opposite, this dataset provides these. The dataset comprises 120 photovoltaic and 273 wind power plants with distinct sides all over Germany from 500 days in hourly resolution. This large number of available sides allows forecasting experiments to include spatial correlations and run experiments in transfer and multi-task learning. It includes side-specific, power source-dependent, non-synthetic input features from the ICON-EU weather model. A simulation of virtual power plants with physical models and actual meteorological measurements provides realistic synthetic power measurement time series. These time series correspond to the power output of virtual power plants at the location of the respective weather measurements. Since the synthetic time series are based exclusively on weather measurements, possible errors in the weather forecast are comparable to those in actual power data. In addition to the data description, we evaluate the quality of weather-prediction-based power forecasts by comparing simplified physical models and a machine learning model. This experiment shows that forecasts errors on the synthetic power data are comparable to real-world historical power measurements.

==> Synthetic Photovoltaic and Wind Power Forecasting Data/acronyms.tex <==
% see https://en.wikibooks.org/wiki/LaTeX/Glossary
\newacronym{lasso}{LASSO}{least absolute shrinkage and selection operator}
\newacronym{nwp}{NWP}{numerical weather prediction}
\newacronym{ml}{ML}{machine learning}
\newacronym{svr}{SVR}{support vector regression}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{mlp}{MLP}{multi-layer perceptron}
\newacronym{gbrt}{GBRT}{gradient boosting regression tree}
\newacronym{mae}{MAE}{mean absolute error}
\newacronym{rmse}{RMSE}{root mean squared error}
\newacronym{nrmse}{nRMSE}{normalized root mean squared error}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{kld}{KLD}{Kullback-Leibler Divergence}
\newacronym{pv}{PV}{photovoltaic}
\newacronym{wrt}{w.r.t.}{with respect to}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{mtl}{MTL}{multi-task learning}
\newacronym{stl}{STL}{single-task learning}
\newacronym{sps}{SPS}{soft parameter sharing}
\newacronym{hps}{HPS}{hard parameter sharing}
\newacronym{csn}{CSN}{cross-stitch network}
\newacronym{sn}{SN}{sluice network}
\newacronym{ern}{ERN}{emerging relation network}
\newacronym{nlp}{NLP}{natural language processing}
\newacronym{lstm}{LSTM}{long-tem short memory}
\newacronym{tcn}{TCN}{temporal convolution network}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{tl}{TL}{transfer learning}
\newacronym{dtw}{DTW}{dynamic time warping}
\newacronym{elbo}{ELBO}{expected lower bound}
\newacronym{csge}{CSGE}{coopetitive soft gating ensemble}
\newacronym{ae}{AE}{autoencoder}
\newacronym{cnnae}{CAE}{convolutional autoencoder}
\newacronym{vae}{VAE}{variational autoencoder}
\newacronym{dae}{DAE}{denoising autoencoder}
\newacronym{pca}{PCA}{principal component analysis}
\newacronym{rl}{RL}{representation learning}
\newacronym{sgd}{SGD}{stochastic gradient decent}
\newacronym{ttl}{TTL}{transductive transfer learning}
\newacronym{itl}{ITL}{inductive transfer learning}
\newacronym{sqtl}{SQTL}{sequential transfer learning}
\newacronym{aic}{AIC}{Akaike information criterion}
\newacronym{bic}{BIC}{Bayesian information criterion}
\newacronym{bma}{BMA}{Bayesian model averaging}
\newacronym{elm}{ELM}{exterem learning machine}
\newacronym{belm}{BELM}{Bayesian exterem learning machine}
\newacronym{relu}{ReLU}{Rectified Linear Unit}
\newacronym{DBN}{DBN}{deep belief network}
\newacronym{RBM}{RBM}{restricted Boltzmann machines}
\newacronym{RBF}{RBF}{radial-basis function}
\newacronym{blr}{BLR}{Bayesian linear regression}
\newacronym{sp}{SP}{source parameters}
\newacronym{crps}{CRPS}{continuous ranked probability score}
\newacronym{ghi}{GHI}{global horizontal irradiance}
\newacronym{dni}{DNI}{direct normal irradiance}
\newacronym{dhi}{DHI}{diffuse horizontal irradiance}
% \newacronym{iconeu}{ICON-EU}{European nest of the global icosahedral nonhydrostatic forecasting model of the German weather service}
\newacronym{iconeu}{ICON-EU}{Icosahedral Nonhydrostatic-European Union}
\newacronym{synop}{SYNOP}{surface synoptic observation}

==> Synthetic Photovoltaic and Wind Power Forecasting Data/experiments.tex <==

\section{Experimental Results}\label{sec_experimental_results}
% Typical forecast errors for wind da-ahead forecasting problems are between 
The following section conducts an experiment that serves as the baseline for future research.
Moreover, the experiment allows comparing forecast errors of the proposed synthetic dataset with real-world forecast errors, showing our dataset's applicability for future research in renewable power forecasts.
% we assess the forecast error with the current state-of-the-art for day-ahead forecasts problem to evaluate if the forecast error is realistic compared to real-world data.
We evaluate physical forecasting techniques on the introduced datasets within the following experiment.
Physical approaches are essential as they are typically utilized when only limited data is available for training.
At the same time, there is an increasing interest in providing high-quality forecasts through~\ac{ml} models even with limited data.
Therefore, we compare the results of physical models with the \ac{gbrt}.
We choose the \ac{gbrt} here as it generalizes well with a limited amount of data and is known to mitigate the effects of overfitting.


To assess the forecast quality of the~\ac{gbrt} concerning reduced data, as it is common with~\ac{tl}, we limit the training data to the last $7$,$14$,$30$,$60$ or $90$ days of training data of a season.
Respectively, we repeat this experiment for each season's different number of training data to ensure that results account for seasonal patterns.
To increase the number of training data within this scenario, we linearly interpolate the data to have a $15$-minute resolution.
Additionally, we make one experiment where we consider the complete training data, indicated through $365$, and compare those forecast errors with an example from real-world datasets.
We consider time steps with the test flag as test data and the remaining data as training data.

Most often the forecast error, in renewable power forecast, is determined by the~\ac{nrmse} given by
\begin{equation}\label{eq_nrmse}
    \text{nRMSE} = \sqrt{\frac{1}{N}\sum_{i=0}^{i=N}{(y_i-\hat{y}_i)^2}},
\end{equation}
where $y_i$ is the $i$-th normalized response from the target and $\hat{y}_i$ is the prediction from a source model on the target.
Note that in the context of renewable power forecasts, we normalize the response $y_i$ by the nominal power to assure comparability of the error for different parks.
To express an improvement of one model over another model we utilize the skill given by
\begin{equation}
    \text{Skill} = \text{nRMSE}_{gbrt}-\text{nRMSE}_{phy},
\end{equation}
where $\text{nRMSE}_{gbrt}$ is the \ac{nrmse} of the~\ac{gbrt} model and $\text{nRMSE}_{phy}$ of the physical model, respectively.
Consequently, values below zero indicate an improvement of the~\ac{gbrt} over a physical forecasting technique.

We optimize the~\ac{gbrt} for each park, season, and number of training data through a grid search by three-fold cross-validation based on the available training data.
Thereby, the learning rate is evaluated at $[\SI{e-6}, \num[round-precision=1]{3.1e-6}, \ldots,\num[round-precision=1]{3.1e-1}, 1]$.
The number of estimators is $300$ and the maximum depth is one of $[2,4,6,8]$.
Other values are the default ones of scikit-learn~\footnote{\url{https://scikit-learn.org/}, Version 0.24, accessed 2022-02-28}.

We utilize the same parametrization for the physical models for creating the power measurements.
The only difference is that we now use the direct radiation and wind speed, respectively, from the~\ac{nwp} as input.
The physical model for the wind dataset is indicated through \textit{Enercon} in the following and \textit{PV Physical} for the~\ac{pv} dataset.
Additionaly, for the wind dataset, we compare the~\ac{gbrt} results with empirical \textit{McLean} power curves~\cite{Mclean2008}.
This power curve is well known and considers typical influences by different terrains.

PV day-ahead power forecasting problems often have an~\ac{nrmse} between $0.06$ and $0.12$~\cite{Schreiber2020Prophesy}.
The mean~\ac{nrmse} values of the PV baseline is at $0.085$ on the proposed synthetic dataset, see Tbl.~\ref{tbl_results_pv}.
Forecast errors of the~\ac{gbrt} model are between $0.12$ and $0.072$ depending on the amount of available training data.
With an increasing amount of training data, the forecast error reduces for this model.
The mean forecast error of the~\ac{gbrt} is only better with the complete training data.
Fig.~\ref{pvsyn_physical_skill_phyiscal} shows the evaluation concerning the skill for the PV dataset.
Up to $14$ days of training data, the~\ac{gbrt} model has substantial positive outliers of the skill.
With additional training data, this effect reduces. 
Beginning from $60$ days of training data, the median skill is close to zero, indicating the~\ac{gbrt} is as good as the physical baseline in most cases.
With $90$ days of training data and the complete dataset, the~\ac{gbrt} has improvements over the physical baseline.

\begin{table}[tb]
    \centering
    \caption{Mean nRMSE values of the~\ac{gbrt} across all available parks for different amounts of training data in comparison to physical models for the PV dataset. Best values for the amount of training data are highlighted in bold.}\label{tbl_results_pv}
    \begin{tabular}{lrr}
    \toprule
    {} &   GBRT &  PV Physical \\
    Number of Days &        &             \\
    \midrule
    7               &  0.120 &       \textbf{0.085} \\
    14              &  0.107 &       \textbf{0.085} \\
    30              &  0.092 &       \textbf{0.085} \\
    60              &  0.089 &       \textbf{0.085} \\
    90              &  0.086 &       \textbf{0.085} \\
    365             &  \textbf{0.072} &       0.085 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[tb]
	\centering
	\includegraphics[width=\textwidth]{images/skill_PVSYN}
	\caption{Skill between the GBRT model and the physical baseline of the dataset for the PV dataset. Values below zero indicate an improvement of the GBRT over the physical reference.}\label{pvsyn_physical_skill_phyiscal}
\end{figure}
% TODO wir koennten hier die fehler bzw. die verteilungen der fehler auch mit realen daten von enercast vergleiche, damit koennten wir begreunden dass der datensatz realistisch ist

Tbl.~\ref{tbl_results_wind} summarizes the mean~\ac{nrmse} for the wind dataset.
The Enercon baseline has a mean~\ac{nrmse} of $0.21$.
Wind day-ahead power forecasting problems typically have an~\ac{nrmse} between $0.1$ and $0.2$~\cite{Schreiber2020Prophesy}.
Depending on the utilized empirical McLean power curve, forecast values of this approach range between $0.212$ and $0.228$.
The~\ac{gbrt} forecasting technique has the best mean~\ac{nrmse} for all numbers of available training data.
With seven days of training data, the~\ac{gbrt} has an~\ac{nrmse} of $0.196$, with $90$ days of training data a~\ac{nrmse} of $0.147$, and with the complete data, an error of $0.125$.
The improvements of the~\ac{gbrt} over the other models are also given through the skill in Fig.~\ref{windsyn_physical_skill_phyiscal}.
In contrast to results from the~\ac{pv} dataset, the median skill is below zero already with seven days of training data.
However, with less than $30$ days of training data, substantial outliers are present compared to the Enercon baseline.
These are not present with more than $30$ days of training data.


All in all, we can observe that the forecast error of the physical baseline and, in particular, errors from the~\ac{ml} technique are comparable to those given by real-world power measurements.
For the~\ac{pv} dataset, we see that the physical baseline is robust, especially in the case of limited data.
At the same time, these excellent results also relate to the fact that the exact physical characteristics are given, which is most often not the case in real-world forecasting problems.
In the case of the proposed wind dataset, the~\ac{gbrt} provides a strong baseline for future research.
In a comparison of those two datasets, the physical approach for the~\ac{pv} dataset considers more physical characteristics in comparison to the Enercon baseline.
At the same time, the~\ac{pv} power forecasting problem can be considered more linear in contrast to wind power forecasts, which makes it easier to model all dependencies within a physical baseline.
Interestingly, errors of the \textit{McLean-Upland} empirical power curve are close to that of the Enercon baseline.
This observation lets us conclude that it is a suitable baseline for limited data when a wind turbine's physical characteristics are not given.

% \textbf{wind observation}
% \begin{itemize}
%     \item mit 30 tagen keine ausreiser mehr im skill
%     \item bereits mit sieben tagen ist der mittere nrmse besser als aller physiklaischer modelle
%     \item enercon ist besonders geeignet da es die realen parameter benutzt
%     \item insbesondere mclean upland sehr nah an dem enercon fehler, welches zeigt, dass die emprische kurve auch gut nutzbar als referenz ist wenn keine physikalischen eigenschaften gegeben sind.
% \end{itemize}


\begin{table}[tb]
    \centering
    \caption{Mean nRMSE values of the~\ac{gbrt} across all available parks for different amounts of training data in comparison to the physical model and different McLean power curves for the wind dataset. Best values for the amount of training data are highlighted in bold.}\label{tbl_results_wind}
    \begin{tabular}{lrrrrrr}
    \toprule
    {} &   GBRT &  Enercon &  McLean- &  McLean- &  McLean- &  McLean- \\
    {} &    &   &  Lowland &  Lowland-Regulated &  Offshore &  Upland \\
    Number of Days &        &          &                &                              &                 &               \\
    \midrule
    7               &  \textbf{0.196} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    14              &  \textbf{0.178} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    30              &  \textbf{0.156} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    60              &  \textbf{0.154} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    90              &  \textbf{0.147} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    365             &  \textbf{0.125} &    0.210 &          0.228 &                        0.216 &           0.239 &         0.212 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[tb]
	\centering
	\includegraphics[width=\textwidth]{images/skill_WINDSYN}
	\caption{Skill between the GBRT model and the physical baseline (Enercon) and different McLean power curves for the wind dataset. Values below zero indicate an improvement of the GBRT over those references.}\label{windsyn_physical_skill_phyiscal}
\end{figure}
